A Survey of Motion Planning and Control Techniques for Self-driving Urban Vehicles

Self-driving vehicles are a maturing technology with the potential to reshape mobility by enhancing the safety, accessibility, efficiency, and convenience of automotive transportation. Safety-critical tasks that must be executed by a self-driving vehicle include planning of motions through a dynamic environment shared with other vehicles and pedestrians, and their robust executions via feedback control. The objective of this paper is to survey the current state of the art on planning and control algorithms with particular regard to the urban setting. A selection of proposed techniques is reviewed along with a discussion of their effectiveness. The surveyed approaches differ in the vehicle mobility model used, in assumptions on the structure of the environment, and in computational requirements. The side-by-side comparison presented in this survey helps to gain insight into the strengths and limitations of the reviewed approaches and assists with system level design choices.

==> IEEEtran/README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************


==> section_mp-motion-primitives.tex <==
\subsection{Motion Primitives}

% From LaValle's RRT paper: The steering problem has received
% considerable attention in recent years.  The task is to compute an
% open-loop trajectory that brings a nonholonomic system from an
% initial state to a goal state without the presence of obstacles.
% Given the general difficulty of this problem, most methods apply to
% purely kinematic models (i.e., systems without drift or momentum).
% For a kinematic car that has a limited turning radius and moves
% forward only, it was shown that the shortest path between any two
% configurations belongs to one of a family of six kinds of curves
% comprising straight lines and circular arcs (Dubins 1957).  For a
% car that can move forward or backward, optimal solutions comprising
% 48 curve types have been obtained (Boissonnat, Cérézo, and Leblond
% 1994; Reeds and Shepp 1990; Sussman and Tang 1991). For more
% complicated kinematic models, nonoptimal steering techniques have
% been introduced, which include for example a car pulling trailers
% (Murray and Sastry 1993) and fire trucks (Bushnell, Tilbury, and
% Sastry 1995).  Techniques also exist for general system classes,
% such as nilpotent (Laffierriere and Sussman 1991), differentially
% flat (Murray, Rathinam, and Sluis 1995; Fliess et al. 1993), and
% chained form (Bushnell, Tilbury, and Sastry 1995; Murray and Sastry
% 1993; Struemper 1997).  For systems with drift and/or obstacles, the
% steering problem remains a formidable challenge.


% In this section we discuss methods for generating feasible paths and
% trajectories for car-like vehicles assuming absence of obstacles.

% Introducing motion primitives as open-loop trajectories
Computing an open-loop trajectory over a relatively short period of
time is the core function used by an overwhelming majority of planning
algorithms.
%
In the case of autonomous cars, these open-loop trajectories often
correspond to maneuvers that are easy to describe, for example,
driving straight, turning left or right, changing lanes, and so on.
%
Due to their atomic nature, these maneuvers are generally called
\emph{motion primitives.}
%
Typically, motion planning algorithms compose motion primitives over
the course of planning time into complex vehicle trajectories.

% 
The choice of motion primitives is a trade-off between the quality of
composed trajectories and the time it takes for a planning algorithm
to find a solution.
%
For this reason, it is important to choose a small but diverse set of
motion primitives.
%
Several possibilities have been previously proposed for car and
car-like vehicle navigation.

%
% Introducing motion primitives:
% * discrete time model;
% * motion between lattice points;
% * Cross-entropy motion planning;
% * optimal curves (Reeds-Shepp, Dubins, Mason Balkom)
% 
%

\paragraph{Constant steering primitives}

%
Intuitive approach for deriving motion primitives uses forward in time
system simulations while applying an analytic function as a control
signal over a fixed period of time.
%
In this case, the global car motion follows a trajectory that
corresponds to a piecewise analytic control signal.
%
Despite superficial resemblance with basis functions presented in
Section~\ref{sec:variational-methods}, motion primitives are
concatenated over planning horizon rather than scaled and
superimposed.
%
This difference facilitates the ``Computer Science'' approach to the
planning problem, in which the solution trajectory is found within a
language formed from an alphabet of all available primitives.
%, which is not a vector space spanned by these primitives.

%
The most basic example of constant steering primitives for a car-like
robot consists of three control input signals: sharp left and right
turns and driving straight.
%
It follows from \cite{reeds1990optimal} that optimal curves can be
approximated by combining such primitives, which are defined over
decreasingly small time intervals.
%
However, this set of primitives is not rich enough to define smooth
car trajectories.


Piecewise continuously differentiable curves for Dubins dynamics can
be obtained if control signal is Lipschitz continuous.
%
In this case, primitives are the following: initiate left and right
turns, continue turning left and right, straighten trajectory, and
drive straight.
%
Also, it is required to use transition primitives between sharp turns
and driving straight.
%
These transition primitives were characterized in
\cite{fleury95primitives}, where they are referred as
\emph{clothoids.}

\paragraph{Lattice-generating primitives}

Two paths that correspond to different strings of motion primitives
may eventually arrive to the same configuration in $\mathcal{X}$.
%
Such situations are common even if the set of motion primitives is
very small.
%
For example, consider basic constant-control primitives presented
above: two strings, left-right-straight and straight-left-right, yield
trajectories that terminate at the same configuration if the initial
positions are identical.
%
Thus, checking both trajectories for satisfying the goal condition is
redundant.


Lattice-based planners tackle this problem by considering motion
primitives that are guaranteed to generate trajectories between
lattice points in the state space.
%
Lattice-generating primitives have been proposed for various car-like
models, such as, mars rovers, Dubins car and Reeds-Shepp
car~\cite{knepper06high, pivtoraiko2009differentially}.
%
For driverless cars, these methods are often used to plan a path
through unstructured environments, such as parking lots, unknown
intersections, and so on \mynote{TODO: include references from DARPA
  challenges}.

\paragraph{Path diversity}

The difficulty with lattice-base planners is in that the resulting
trajectories often \emph{chatter} between two or more primitives to
attain ``average'' behavior.
%
Some recent work has been aimed at improving path diversity while
maintaining low complexity of primitives~\cite{branicky08path}.
%
In this work, a path diversity is characterized based on correlation
function of collision probabilities.
%
Since such a correlation function is difficult to compute, the set of
diverse path were generated for Dubins car using an approximation of
this function.
%
The results illustrate that using the proposed heuristic function it
is possible to improve significantly path diversity while considering
only one percent of the initial path set.


\paragraph{Learning Primitives from Expert Input}


Human expertise can aid planning algorithms in computing complex
trajectories that would be otherwise outside of the domain of
concatenated motion primitives.
%
To this end, expert inputs have been mapped using high-precision
instruments during maneuver execution, such as, for example,
pendulum-turn and trail-braking maneuvers, which are commonly used in
rally racing~\cite{velenis07aggressive, velenis07modeling}.
%
Using these maneuvers as motion primitives enriches the set of
attainable trajectories while reducing the amount of primitives that
achieve a desired solution to a minimum.

\paragraph{Boundary value problem---unifying approach}

A substantially more systematic way for constructing motion primitives
uses boundary value problem (BVP) solvers.
%
BVP can be posed as an optimal planning problem by dropping collision
avoidance constraints.
%
In this case, many trajectory optimization algorithms, discussed in
Section~\ref{sec:variational-methods} can be used to find a numerical
solution.
%
Contrary to variational methods, however, BVP solutions are not
intended to provide a globally feasible trajectory, rather they are
used as primitives to build one.

Computing BVP solutions between lattice points in the configuration
space generates primitives for lattice planners.
%
Using system symmetries, it is possible to extend a finite set of
primitives generated at the origin to the entire infinite lattice.

In many cases, trajectory optimality guarantees the uniqueness of a
maneuver between two points. However, optimality condition can be
dropped in favor of simplifying the control signal for primitives.
%
Such an approach is proposed in \cite{murray1993nonholonomic}, where
suboptimal trajectories for nonholonomic chained systems have been
generated between any two using just sinusoids.
%
This analytic forms require significantly less memory to store
compared with traditional collocation discretization.


